The range of geometrical frustration in lattice spin models

The concept of geometrical frustration in condensed matter physics refers to the fact that a system has a locally preferred structure with an energy density lower than the infinite ground state. This notion is however often used in a qualitative sense only. In this article, we discuss a quantitative definition of geometrical frustration in the context of lattice models of binary spins. To this aim, we introduce the framework of local energy landscapes, within which frustration can be quantified as the discrepancy between the energy of locally preferred structures and the ground state. Our definition is scale-dependent and involves an optimization over a gauge class of equivalent local energy landscapes, related to one another by local energy displacements. This ensures that frustration depends only on the physical Hamiltonian and its range, and not on unphysical choices in how it is written. Our framework shows that a number of popular frustrated models, including the antiferromagnetic Ising model on a triangular lattice, only have finite-range frustration: geometrical incompatibilities are local and can be eliminated by an exact coarse-graining of the local energies.

==> FLS_table.tex <==
\renewcommand\tabularxcolumn[1]{m{#1}}
\newcolumntype{x}[1]{>{\raggedright}m{#1}}
\begin{table*}[p]
  \centering
\caption{ The FLS model. }
  \setlength{\tabcolsep}{10pt}
  \label{tab:FLS} 
  \begin{tabularx}{\textwidth}{cm{1cm}m{2.5cm}ccccc}
    \textbf{ID} & \textbf{FLS}  & \textbf{Ground state} & $E_0$ &  & $f_7$ &  $f_{10}$ &  $f_{13}$ \\
    \hline
    \input{FLS_data}
\end{tabularx}
\end{table*}

